Exact Penalty Method for Variationally Coherent Stochastic Programming Problems

The paper concerns optimization problems with general equality and inequality constraints and with constraints expressed by a convex set. In order to solve these problems, the general constraints are treated by an exact penalty functions while the others by mirror descent approach. The paper introduces a constraint qualification condition under which the solution of the optimization problem with an exact penalty function and constraints defined by the convex set is a solution of the original problem with constraints. The paper extends results on exact penalty functions to the case when together with general equality and inequality constraints additional constraints defined by a convex set are present. In order to solve the optimization problems with exact penalty functions, a mirror descent algorithm is proposed. It is assumed that instead of using gradients of functions defining constrained optimization problems, their stochastic approximations can be applied. The paper establishes global convergence of the proposed method under the assumption that applied exact penalty functions lead to variationally coherent optimization problems. Since exact penalty functions are not differentiable, the concept of variationally coherent problems is extended to the problems defined by functions exhibiting Clarke's generalized gradients. The behavior of the proposed method is illustrated by some numerical examples.

==> binary_spectral_embeddings.tex <==
\subsection{Binary Spectral Graph Embeddings}

The next application of our method are binary graph embeddings. Given an undirected graph $G$ with $N \in \N$ vertices, the aim is to construct a representation of each vertex in $\{-1, 1\}^k$, such that it minimizes the overall distance between connected vertices
\begin{align}
\minimize_{x \in [-1, 1]^{N \times K}} \quad
    & \sum_{i \in [N]}\sum_{j \in [N]} A_{i,j}\norm{x_i - x_j}^2    \label{binary-objective}  \\
\subjectto \quad 
    & \norm{x_{i,k}}^2  = 1, \quad i \in [N],\ k \in [K]            \label{binary-cube} \\
    & \frac{1}{N} x^T x = I                                         \label{binary-orthogonal}
    % & g_j(x) \leq 0, \quad j \in I       \label{binary-cube-constraints} \\
\end{align}
where the matrix $A$ is the adjacency matrix of the graph $G$ and $i$-th row of the matrix $x$ is the representation of $i$-th vertex. The above problem is a direct modification of the spectral embedding problem, where the constraint (\ref{binary-cube}) is being replaced with $\norm{x_{\cdot, k}} = 1$ for all $k \in [N]$. In such a case, the problem is equivalent to finding $K$ eivenvectors of the Laplacian matrix $L$ with the smallest eigenvalues.


\paragraph{Existence of the solution.}
For the feasible set to be non-empty, we assume that $N$ is divisible by $2^K$. Otherwise, the orthogonality constraint (\ref{binary-orthogonal}) would be violated. For $K > 1$ and $N$ being odd, no two binary vectors $x, y \in \{-1, 1\}^N$ could be orthogonal, since for $x^Ty = 0$ to hold, the vector $y$ must differ from $x$ at exactly $N/2$ coordinates. Applying this argument recursively, we obtain that $N$ being divisible by $2^K$ implies there exists at least $K$ orthogonal binary vectors.

Because there are few orthogonal binary vectors, we perturb our problem to the following
\begin{align}
\minimize_{x \in [-1, 1]^{N \times K}} \quad
    & \sum_{i \in [N]}\sum_{j \in [N]} A_{i,j}\norm{x_i - x_j}^2    \label{rel-binary-objective}  \\
\subjectto \quad 
    & \norm{x_{i,k}}^2  = 1, \quad i \in [N],\ k \in [K]            \label{rel-binary-cube} \\
    & \frac{1}{N}x^T x + s = I                                      \label{rel-binary-orthogonal} \\
    & -C \leq s \leq C
    % & g_j(x) \leq 0, \quad j \in I       \label{binary-cube-constraints} \\
\end{align}

\subsection{Embedding via main binary components}

\begin{definition}[Laplacian Matrix] Let $G = (V, E)$ be an undirected graph with $n \in \N$ vertices, $A \in \{0, 1\}^{n \times n}$ be its adjacency matrix. The Laplacian matrix $L \in \Z^{n \times n}$ is defined as:
\begin{equation}
    L = D - A
\end{equation}
where $D = \diag{\{\deg(v_k)\}^N_{k=1}}$ is a diagonal matrix of degrees of vertices.
\end{definition}

\begin{definition}[Spectral Embedding]
Let $G = (V, E)$ be an undirected graph with $n \in \N$ vertices. Spectral embedding of size $k \in \N$ of the graph $G$ is a matrix $x \in \R^{n \times k}$ is defined as the solution to the following optimization problem
\begin{align}
\minimize_{X \in \R^{n \times k}} \quad
    & \sum_{i = 1}^n\sum_{j = 1}^n A_{i, j}\norm{X_i - X_j}^2 
    = \tr{X^T L X}  \label{spectral-objective}    \\
\subjectto \quad 
    & X^T X = I     \label{spectral-orthogonal}
    % & \norm{x_{\cdot,k}}^2  = 1 ,\ k \in [K]  \label{spectral-cube} \\
    % & g_j(x) \leq 0, \quad j \in I       \label{binary-cube-constraints} \\
\end{align}
where $X_{\cdot,k} \in \R^n$ denotes $k$-th column of the matrix $X$ and $L$ is the Laplacian matrix of the graph $G$.
\end{definition}

\begin{proposition}[Spectral Embeddings as Eigenvectors]
The solution to the spectral embedding problem are $k$ eigenvectors of the Laplacian matrix $L$ with the smallest eigenvalues.
\end{proposition}

The eigenvectors with the smallest eigenvalues can be computed consecutively. In such a case, a new eigenvector must additionally be orthogonal to the former ones.

To find $k$-th eigenvector with the smallest eigenvalue, we can solve the following problem:
\begin{align}
\minimize_{x \in \R^{n}} \quad
    & \sum_{i = 1}^n\sum_{j = 1}^n A_{i, j}\norm{x_i - x_j}^2 
    = x^T L x  \label{spectral-objective}    \\
\subjectto \quad 
    & X^T x = 0 \label{spectral-step-orthogonal} \\
    & \norm{x} = 1 \label{spectral-step-norm}
\end{align}
where $X \in \R^{n \times k-1}$ is a matrix of previously found eigenvectors. 

In practice, for large sparse adjacency matrices typical for learning graph embeddings, the solution can be achieved via simple iterative procedure, and the orthogonality constraint (\ref{spectral-step-orthogonal}) can be realised via projection on the subspace.

In binary setting, additional problems appear. The problem is not necessarily decomposable into a sequence of consecutive problems of finding the best fitting vector, orthogonal to the previous ones.








% \begin{proof} The trace of a matrix is the sum of its eigenvalues. Hence, the aim is to find an orthogonal system $X$, such that $X^T L X$ has the smallest sum eigenvalues. $L$ is positive semi-definite matrix, since $G$ is undirected and the adjacency matrix $A$ is symmetric, hence we can spectrally decompose $L$ into $U\diag{\lambda}U^T$. Then it follows that:
% \begin{equation}
%     X^T L X = X^T U \diag{\lambda} U^T X = Z^T \diag{\lambda} Z
% \end{equation}
% where $Z \in \R^{n \times k}$ has orthonormal columns, since it is a product of orthonormal matrix $X$ and orthonormal matrix $U$. Later, we minimize the trace, which is
% \begin{equation}
%    \tr{Z^T \diag{\lambda} Z} = \sum_{i = 1}^n \lambda_i Z_i^T Z_i
% \end{equation}
% \end{proof}
